Scaling down an insect-size microrobot, HAMR-VI into HAMR-Jr

Here we present HAMR-Jr, a \SI{22.5}{\milli\meter}, \SI{320}{\milli\gram} quadrupedal microrobot. With eight independently actuated degrees of freedom, HAMR-Jr is, to our knowledge, the most mechanically dexterous legged robot at its scale and is capable of high-speed locomotion (\SI{13.91}{bodylengths~\second^{-1}}) at a variety of stride frequencies (\SI{1}{}-\SI{200}{\hertz}) using multiple gaits. We achieved this using a design and fabrication process that is flexible, allowing scaling with minimum changes to our workflow. We further characterized HAMR-Jr's open-loop locomotion and compared it with the larger scale HAMR-VI microrobot to demonstrate the effectiveness of scaling laws in predicting running performance.

==> notes.tex <==
--------------------------------------------
Toward Autonomy in Sub-Gram Terrestrial Robots
https://www.annualreviews.org/doi/full/10.1146/annurev-control-053018-023814
 
 -millirobots (defined here as robots with a mass of less than 1 g; microrobots are defined as robots with a mass of less than 1 mg)

-Survivors after an earthquake could be found more quickly if robotic bugs could target the efforts of first responders ... manufacture large structures ... minimize surgical interventions ...inform insect biomechanics research 

(LARGE EXCEL WITH SPECS FOR ROBOTS!!):
the entire database of robots evaluated is available at http://ter.ps/botsandbugs.

Adding legs or compliance can allow for improved locomotion abilities while still tethered.

-absolute speed is generally proportional to body length.

-empirical scaling law from Rubin et al. (62), which is based on data from fast-moving organisms across scales and generally represents an upper bound for speed performance in biology. Even the top robotic performers are approximately an order of magnitude below this cap, and the majority are closer to three orders of magnitude below, indicating that substantial improvements can still be made in the performance of small-scale robots.

-two metrics for power autonomy: the energy required to move 1 m and the cost of transport (COT)

-energy needed to move 1 m does not decrease dramatically with decreasing size (either mass or characteristic length) among insects. Lower efficiencies in smaller animals

- energy required by robots for locomotion is still orders of magnitude higher than the energy required by similarly sized insects at scales below 1 g. This shows an efficiency gap between the robotic systems and insects and points toward research opportunities to understand the energetic losses in both mechanical design and actuation.

key areas that lead toward insect-level autonomy—power autonomy (two metrics dependent on both the energy source and the robot design: mass-specific run time and robot recharging), mobility autonomy(step height, gap size, and traversal probability), and control autonomy (ability to sense the environment, path deviation, obstacle avoidance, and path length to goal)

------------------------------------------

A 5mg micro-bristle-bot fabricated by two-photon lithography

-first demonstration of a microbristle-bot, with 3D-printed legs, fabricated by two-photon polymerization (TPP) lithography

-5 mg, in the size of 2 mm × 1.87 mm × 0.8 mm, and can achieve a speed up to 4 times the body length per second.

-resonant frequency around 6.3 kHz, which can be tailored based on their geometry

-Another microrobot shown in [11] with 1.5 mm × 0.7 mm × 0.2 mm dimensions utilizes kicks from a pair of legs with different resonant frequencies powered by vibrations.

-net horizontal movement of a bristle-bot is achieved by the modulation of frictional force due to oscillations of the normal force from vertical displacement of piezoelectric shaker, leading to a stick-slip motion of their legs


-------------------------------------------

Models and the scaling of energy costs for locomotion

-mechanical cost of transport for running
[power/(body mass  speed)] will be independent of body mass; but measurements of oxygen consumption for
running birds and mammals show that the metabolic cost
of transport is proportional to (body mass)−

-efficiency seems to increase with body mass, at least in running and flight, is discussed in relation to the metabolic energy costs 

-For animals running in dynamically similar fashion, all forces are proportional to body weight and all velocities to the speed of running. Thus mechanical power is proportional to (weight  speed), and the mechanical cost of transport [power/(mass  speed)] is independent of body mass. Alexander (1977) showed that cost of transport was independent of mass for specific models of walking and running

- muscles do the work of locomotion more efficiently in larger animals

-The most urgent need, however, in studies of the scaling of energy costs in locomotion, is for better understanding of the relationship between mechanical work and metabolism

-Hill’s Equation, derived from isotonic experiments, does not predict forces in work loops well


-------------------------------------------

Designing minimal and scalable insect-inspired multi-locomotion millirobots

-ten-gram palm-sized prototype—the smallest
and lightest self-contained multi-locomotion robot reported so far—by folding a quasi-two-dimensional metamaterial18 sandwich formed of easily integrated mechanical, material and electronic layers,

Tribot is a three-legged robot with dimensions
of 30 mm (width), 58 mm (length) and 58 mm (height) with ...three linear spring-type
shape-memory alloy (SMA) actuators that function as ‘muscles

jumps to a height of 140.6 mm on average (almost 2.5 times the robot’s
height) from the edge

robot’s horizontal distance jump for a trigger
power of 3.7 W (Fig. 2b) and 2.7 W, and with an added payload of 5 g...the average jumping distance was 230 mm (almost four times its body length)

-------------------------------------------

Insect-scale fast moving and ultrarobust soft robot

-a curved unimorph piezoelectric structure whose relative speed of 20 body lengths per second is the fastest measured among published artificial insect-scale robots.

-Under an alternating current (AC) driving power near the resonant frequency (850 Hz) of the structure, a prototype 10-mm-long robot (0.024 g) attained a relative speed of 20 BL/s

-move smoothly carrying a load
weighing 0.406 g, which is six times heavier than that of the robot; 

- prototype 3 cm–by–1.5 cm robot

- 25-mm-long prototype robot w...the trial with the fastest speed at 8.7 cm/s at 200 Hz 

-For animals including both mammals (purple) and arthropods (orange), relative speeds show a strong negative scaling law with respect to the body mass, showing that relative running speeds increase as body masses decrease.

- Using a prototype 30-mm-long robot operating at 140 Hz ... cost of transport (COT) of the robot was about 14 (section S5), the lowest reported COT for robots and insects below 1 g (fig. S11) (46–59) with a relative speed of 4 BL/s under a power of 0.343 mW.

- robustness of the prototype soft robot was demonstrated by applying a 100-g mass (1500 times its own body weight) with little change in its speed after the mass was removed

-carry loads equal to the weight of a peanut (0.406 g)
(Fig. 5, F and G). The robot was able to move smoothly while carrying a load that is six times its own weight at about one-sixth of the
original speed

-slope climbing capability of the robot is demonstrated in movie S7, in which the robot reached 7 BL/s while climbing a slope with an angle of 7.5° (Fig. 5D) and 1 BL/s while climbing
a slope with an angle of 15.6° (


-------------------------------------------



